QFAST: Quantum Synthesis Using a Hierarchical Continuous Circuit Space

We present QFAST, a quantum synthesis tool designed to produce short circuits and to scale well in practice. Our contributions are: 1) a novel representation of circuits able to encode placement and topology; 2) a hierarchical approach with an iterative refinement formulation that combines "coarse-grained" fast optimization during circuit structure search with a good, but slower, optimization stage only in the final circuit instantiation stage. When compared against state-of-the-art techniques, although not optimal, QFAST can generate much shorter circuits for "time dependent evolution" algorithms used by domain scientists. We also show the composability and tunability of our formulation in terms of circuit depth and running time. For example, we show how to generate shorter circuits by plugging in the best available third party synthesis algorithm at a given hierarchy level. Composability enables portability across chip architectures, which is missing from the available approaches.

==> sections/algorithm.tex <==
\section{Synthesis Algorithm} \label{algorithm}

The goal of this algorithm is to provide a means for decomposing a large unitary into a product of smaller unitaries of a chosen size. Most bottom-up synthesis algorithms directly convert a target unitary into a circuit by building the circuit with gates from the low-level gate set. Our algorithm, however, takes a recursive approach by first converting the unitary into smaller general unitary gates. The size of the smaller gates at each step can be specified. We can then recursively call this algorithm on the smaller unitaries until they are 2-qubit unitaries; in which case, we will use the canonical 2-qubit unitary decomposition.

This algorithm is accomplished by encoding the continuous circuit structure of a fixed length described in the previous section into a classical optimizer. This requires a loss function that represents our distance from the Target unitary $U_T$. Once we have reached a suitable distance, we recursively deconstruct the circuit encoding into the smaller unitaries until we finish. There are two stages to the algorithm, one where we use a large learning rate in the optimizer to quickly find a suitable solution. In the second stage, we refine our results by using a fixed circuit structure and an optimizer set to reduce the loss below a final acceptable threshold.

\subsection{Loss Function}

The goal of the synthesis algorithm is to minimize $\lVert U_C - U_T\rVert$, where the $U_C$ is the operation implemented by the encoded circuit and $U_T$ is the target specification. In exact synthesis, $\lVert U_C - U_T\rVert = 0$ implies a solution, however, we classify our algorithm as approximate. That is, we look to find a $U_C$ that satisfies $\lVert U_C - U_T\rVert < \epsilon$ for some acceptable threshold $\epsilon$.

Most synthesis algorithms use the diamond norm to measure quantum distinguishability, however, this is a very computationally expensive operation. Instead we base our loss function off the Hilbert-Schmidt inner product:

$$\langle U_C, U_T \rangle = Tr(U_C^{\dagger}U_T)$$

The closer that $U_C$ and $U_T$ become the closer that the product $U_C^{\dagger}U_T$ becomes to the identity. As the product approaches the identity, the trace of it becomes closer to the dimension of the matrix. Our completed loss function normalizes the value of the inner product to be within the range of $(0, 1)$. Lastly, we invert it, so that a value of 0 correspondes to an exact match and a value of 1 implies the opposite. The final function is given by:

$$\Delta(U_C, U_T) = \sqrt{1 - \frac{|Tr(U_C^{\dagger}U_T)|^2}{d^2}}$$

Our algorithm has two stages, in the first we use an optimizer with a large learning rate to quickly explore and find a solution. We use an epsilon of 0.02 in the first stage. The refinement step comes after the initial exploration stage. During this second stage, we attempt to refine our loss down to a more acceptable final loss of $10^{-5}$.



\subsection{Recursive Algorithm}

This algorithm is preformed recursively. If we start with a 6-qubit unitary, we might decide to decompose this into a product of 3-qubit unitaries. This algorithm is then recursively applied to each of those 3-qubit unitaries to break them down into 2-qubit unitaries. At this point we can use the canonical 2-qubit decomposition to convert these into native gates. The final circuit is then pieced together. Due to the approximate nature of this algorithm, the error at each stage accumulates when building the final circuit, often resulting in an error greater than $10^{-5}$. We are not too concerned with this due to the fact the state-of-art noisy hardware has error values order's of magnitude greater than this.


==> sections/relatedworks.tex <==
\section{Related Works} \label{sec:works}

\subsection{2-qubit KAK Decomposition}

The 2-qubit canonical decomposition, widely known as the KAK Decomposition \cite{tucci2005introduction}, is a top-down approach to compilation that applies the Cartan decomposition to quantum computing. This decomposition allows one to factor a general 2-qubit operation into a 3-parameter, non-local operation surrounded by local operations. Further work describes how this non-local operation can be quickly decomposed into at most three CNOT gates \cite{vidal2004universal}. Together this makes the KAK decomposition a powerful tool in quantum compilation. This tool has become ubiquitous within quantum compilers for its optimality. It is primarily used in optimization as any string of 2-qubit operations can be resynthesized into at most 3 CNOTs.

IBM’s QISKit transpiler \cite{cross2018ibm} has used this to optimize circuits further by approximating the nonlocal operation with fewer CNOTs than necessary. This presents the quantum approximation trade-off. It is often the case that a circuit can be approximated with fewer gates; in this case, there is a loss due to the approximation but a gain in shorter depth circuits. In the NISQ era, each additional 2-qubit gate comes with a significant noise penalty, as such, it might be worthwhile dropping some in favor of a shorter circuit. We used this transpiler to piece together the unitaries outputted from our algorithm.

\subsection{Generalized KAK Decomposition}

Khaneja and Glaser have applied the KAK Decomposition to more than just 2-qubit systems \cite{khaneja2000cartan}. Their work that applied the Cartan Decomposition to quantum computing also generalized to arbitrary sized systems. This is separated from the previous canonical 2-qubit decomposition, because the generalization is far from optimal. 

\subsection{Quantum Shannon Decomposition}

The Quantum Shannon Decomposition (QSD) \cite{shende2006synthesis} is a recursive algorithm that heavily uses the Cosine-Sine Decomposition (CSD). This is implemented in the UniversalQ Compiler \cite{iten2016quantum}, which is one of the algorithms we evaluated alongside our tool. This is a recursive algorithm that first uses the CSD to convert a unitary matrix into the product of a multi-controlled y-rotation surrounded by two controlled unitaries. Each of these controlled unitaries can then be rewritten into two unitaries surrounding a multi-controlled z-rotation. The algorithm then recurses on the four unitary blocks created. At each level the size of the problem decreases by one qubit, which makes this algorithm exponential in the size of the input. This is why the UniversalQ Compiler results are exponential.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.2]{images/2020-01-05-155001_screenshot.png}
    \caption{Circuit depiction of the Quantum Shannon Decomposition from \cite{shende2006synthesis}. The smaller unitaries on the right hand side act on 1 less qubit than the unitary on the left hand side.}
    \label{fig:gi}
\end{figure}

\subsection{Search Compiler}
The Search Compiler \cite{davis2019heuristics} is a heuristic-based search strategy over the graph of all circuits. This method is being used to compile small circuits with small amounts of error introduced much more efficiently than the Quantum Shannon Decomposition described previously. The author of this method mentions an average of $2.4\times$ average reduction in circuit depth over a compiler using cosine-sine decomposition.

The core idea in the Search Compiler is a canonical representation of a circuit that forms a graph structure. In this circuit representation, a layer of single-qubit rotations are performed on all qubits followed by a single CNOT gate. This structure is then repeated as many times as necessary. This naturally forms a tree structure, where the root node is the first layer of single-qubit rotations. The root node classifies all circuits with no CNOTs. For each possible position of a CNOT gate, there exists a child of the root with a CNOT in that position followed by more rotations. This layer in the tree classifies all circuits with one CNOT.

Using an A* search with the Hilbert-Schmidt inner product as a search heuristic, the search compiler searches over the circuit tree until it finds a suitable circuit. At every node expansion, a classical optimizer is run to find the parameters of the rotations. This process is extremely expensive for two reasons. One, the tree blows up with a branching factor equal to the number of pairs of qubits (assuming an all-to-all connectivity). Two, the use of a classical optimizer is extremely expensive on it's own. This approach does not scale well, taking more than a day to produce a reasonably sized 4-qubit circuit. However, the circuits produced have been shown to be better than hand-optimized circuits for a variety of algorithms.
